Learning-to-Fly: Learning-based Collision Avoidance for Scalable Urban Air Mobility

With increasing urban population, there is global interest in Urban Air Mobility (UAM), where hundreds of autonomous Unmanned Aircraft Systems (UAS) execute missions in the airspace above cities. Unlike traditional human-in-the-loop air traffic management, UAM requires decentralized autonomous approaches that scale for an order of magnitude higher aircraft densities and are applicable to urban settings. We present Learning-to-Fly (L2F), a decentralized on-demand airborne collision avoidance framework for multiple UAS that allows them to independently plan and safely execute missions with spatial, temporal and reactive objectives expressed using Signal Temporal Logic. We formulate the problem of predictively avoiding collisions between two UAS without violating mission objectives as a Mixed Integer Linear Program (MILP).This however is intractable to solve online. Instead, we develop L2F, a two-stage collision avoidance method that consists of: 1) a learning-based decision-making scheme and 2) a distributed, linear programming-based UAS control algorithm. Through extensive simulations, we show the real-time applicability of our method which is $\approx\!6000\times$ faster than the MILP approach and can resolve $100\%$ of collisions when there is ample room to maneuver, and shows graceful degradation in performance otherwise. We also compare L2F to two other methods and demonstrate an implementation on quad-rotor robots.

==> chapters/abstract_old.tex <==
\begin{abstract}
\todo{Abstract is $\leq$200 words! The paper is 6 for free, 8 for gold.}
With increasing urban population densities, there is a global interest in Urban Air Mobility (UAM), where hundreds of autonomous Unmanned Aircraft Systems (UAS) execute missions in the airspace above major cities for moving people and goods. 
The two fundamental safety challenges in UAM are with urban air traffic management and airborne collision avoidance. 
Unlike traditional human-in-the-loop air traffic management, UAM requires decentralized autonomous approaches that scale for an order of magnitude higher aircraft densities and are applicable to urban settings. %and operate along unconstrained paths with free flight.  
We present Learning-to-Fly, a decentralized mission planning and on-demand airborne collision avoidance framework for multiple UAS to execute missions with spatial, temporal and reactive mission objectives while sharing the same airspace for collision-free flight. 
Using Signal Temporal Logic to capture mission specifications, our approach synthesizes trajectories with safety and performance guarantees. 
For on-demand airborne collision avoidance, we develop a two-stage method that consists of: 
1) Learning-based conflict resolution to decide a sequence of maneuvers for the two UAS to execute 
cooperatively avoid potential conflicts arising in the near future, and 
2) CA-MPC, a distributed Model Predictive Control scheme for the two UAS to execute these maneuvers for collision avoidance.
Through extensive simulations, we show the real-time applicability of the supervised learning method for conflict resolution. We also compare its performance to a greedy approach, a randomization-based approach and a Mixed Integer Programming (MIP) based approach. 
Our method is successful in resolving collision over $99\%$ of the time, and with a run-time in milliseconds, which is orders of magnitude faster than the MIP-based approach. 
Learning-to-Fly is demonstrated on real quadrotor drones. 
	
%	With increasing urban population densities, there is a global interest in Urban Air Mobility (UAM), where hundreds of autonomous Unmanned Aircraft Systems (UAS) execute missions in the airspace above major cities for moving people and goods. 
%The two fundamental safety challenges in UAM are with urban air traffic management and airborne collision avoidance. 
%Unlike traditional air traffic management which operates in a centralized manner, UAM requires decentralized approaches that scale for an order of magnitude higher aircraft densities and operate along unconstrained paths with free flight.  
%We present Learning-to-Fly, a decentralized mission planning and on-demand airborne collision avoidance framework for multiple UAS to execute missions with spatial, temporal and reactive mission objectives while sharing the same airspace for collision-free flight. 
%Using Signal Temporal Logic to capture mission specifications, our approach synthesizes trajectories with safety and performance guarantees. 
%For on-demand airborne collision avoidance, we develop a two-stage method that consists of: 
%1) Learning-based conflict resolution to decide a sequence of maneuvers for the two UAS to execute 
%cooperatively avoid potential conflicts arising in the near future, and 
%2) CA-MPC, a distributed Model Predictive Control scheme for the two UAS to execute these maneuvers for collision avoidance.
%Through extensive simulations, we show the real-time applicability of the supervised learning method for conflict resolution. We also compare its performance to a greedy approach, a randomization-based approach and a Mixed Integer Programming (MIP) based approach. 
%Our method is successful in resolving collision over $99\%$ of the time, and with a run-time in milliseconds, which is orders of magnitude faster than the MIP-based approach. 
%Learning-to-Fly is demonstrated on real quadrotor drones. 
\end{abstract}


==> chapters/crazy_exp.tex <==
In order to evaluate the feasibility of the deconflicted trajectories, the trajectories were flown using two Crazyflie quad-rotor robots.  
The two robots representing UAS 1 and UAS 2, respectively, flew 5 trajectories generated using Learning-to-Fly.
The UAS were programmed to execute both the initial conflicting 
trajectories and the deconflicted trajectories.
Pose estimates for the UAS were obtained from using the Vicon motion 
capture system, and recorded. 
Fig. \ref{fig:scen1_w_ca} shows one such trajectory (before and after 
collision avoidance). Learning-to-Fly de-conflicts the trajectories 
in a manner such that the actual quad-rotors can execute them 
successfully. 
Videos of additional experimental recordings and simulations can be found at \url{https://tinyurl.com/yxttq7l5}.


 %Overall, the drones executed the deconflicted trajectories 
 %successfully.
%The two drones representing UAS1 and UAS2, respectively, executed the planned trajectories with waypoints input at $10\,Hz$.
%The drones were programmed to execute both the initial conflicting trajectories and the deconflicted trajectories. 
%The position of the drones were recorded through a Vicon system at a rate of 100Hz and assessed for collision.

%An example of a scenario after deconfliction is shown in  
%Fig. \ref{fig:scen1_w_ca}. 
%As can be seen in Fig. \ref{fig:scen1_w_ca}, CA-MPC deconflicts the intial trajectories and the drone successfully complete the deconflicted trajectories.

 




==> chapters/experimental_setup.tex <==
\subsection{Experimental Setup}
\label{sec:exp_setup}










%A test set of 10K random, conflicting trajectories were generated by 
%using the minimum-jerk trajectory generation algorithm 
%from~\cite{pant2018fly}.
%The time horizon was set to $T=4$s and $dt=0.1$s. Thus, each 
%trajectory consists of $N+1=41$ time-steps. 
%The initial and final waypoints were sampled from the standard normal 
%distribution, initial velocities were set to zero and the 
%collision point was fixed to be $(1,1,1)$. 
%An example trajectory is presented in Fig. \ref{fig:scen1_w_ca}.



==> chapters/outline_overview.tex <==
\subsection{Outline of the paper}

The following section (Section \ref{sec:overview}) presents an overview of the 
framework we develop to solve problems \ref{prob:traj_STL_highlevel} and 
\ref{prob:CA_highlevel}. Section \ref{sec:STL_intro} is an introduction to 
Signal Temporal Logic (STL), which we use for formally representing mission 
requirements. 
Section \ref{sec:problem_planning} presents the variant of the 
algorithm from \cite{pant2018fly} that we use for UAS trajectory generation 
for satisfying STL specifications. 
Section \ref{sec:CA} formalizes the two UAS 
collision-avoidance problem and formulates the solution to it as a 
Mixed-Integer Linear Program (MILP). 
Sections \ref{sec:CA_MPC} and \ref{sec:learning} outlines our approach to the problem, where instead of solving the computationally expensive MILP, we first solve a discrete 
conflict-resolution problem, and then a decentralized and co-operative 
collision avoidance MPC controller. 
These two components form the basis of our framework. 
We present a learning-based approach for the conflict resolution, as well as a greedy, computationally lightweight approach to the problem that serves as a baseline for comparison. 
In Section \ref{sec:experiments} we evaluate our framework for 2 UAS collision avoidance through extensive simulations and compare its performance to the MILP approach and the greedy algorithm. 
Section \ref{sec:casestudy} demonstrates how we combine the trajectory generation method of Section \ref{sec:problem_planning} and the collision avoidance schemes developed in this paper into a UTM framework. 
Finally in Section \ref{sec:future} we discuss potential future directions to overcome the limitations of the current approach.

==> chapters/problemStatement_planning_old.tex <==
\subsection{UAS planning with STL specifications}
\label{sec:problem_planning}

Fly-by-logic, the method of \cite{pant2018fly}, generates trajectories by centrally planning for fleets of UAS with STL mission specifications, e.g. for the specification $\varphi_{\text{reach-avoid}}$ of example \ref{ex:reach_avoid_exmp}. It does by maximizing a smooth approximation ($\srob_\formula$) of the robustness function \cite{pant2017smooth} by picking waypoints (connected via jerk-minimzing splines \cite{MuellerTRO15}) for each UAS through centralized, non-convex optimization.

While the method shows success in planning for multiple multi-rotor 
UAS, its performance degrades as the number of UAS being planned for 
increases. There are two main reasons for this: a) it solves a 
(non-convex) optimization involving the variables of all the UAS, so 
the problem becomes harder as the number of variables increase, and 
b) for $J$ UAS, it has to account for $J \choose 2$ terms for 
pair-wise separation between the UAS (eq. \ref{eq:timed_RA}). So 
increasing the number of UAS makes the problem harder to solve. For 
these reasons, the method cannot be used for real-time planning. In 
addition, for a large airspace with a small number of UAS, centrally 
taking the $J \choose 2$ constraints into account might not be 
necessary as possible collisions between UAS could be possibly 
infrequent. 

Taking these observations into account, we use the underlying optimization of  \cite{pant2018fly} to generate trajectories \footnote{we could also have used the method of \cite{Raman14_MPCSTL}, but instead use \cite{pant2018fly} because of it being computationally faster and tailored for multi-rotor robots.}, but allow each UAS to independently (and in parallel) solve for their own STL specification. This is captured in the following problem:

\begin{myprob}
\label{prob:STLtraj}
For UAS $j$, given STL specification $\varphi_j$, generate trajectory 
$\sstraj_j$ such that $\sstraj_j \models \varphi_j$. 
\end{myprob}


%Each UAS $d$, is given its mission as a STL specification $\phi_d$. This specification is defined over the variables of just UAS $d$, and does not involve any other UAS. An example of such a specification is $\phi_1 = \always_I \neg (p_1 \in \text{Unsafe}) \land \eventually_I (p_1 \in \text{Goal})$, corresponding to a timed reach-avoid problem. Given such a specification a UAS, each UAS $d$ uses the method of \cite{pant2018fly} to generate trajectories that satisfy $\phi_d$:

Each UAS solves this problem (to generate a trajectory of duration 
$hrz(\varphi_j)$) by solving an optimization of the form:

\begin{equation}
\label{eq:single_FbL}
\begin{split}
\text{max}_{\mathbf{w}_j} \,\srob_{\varphi_j}(L\mathbf{w}_j) \\
F\mathbf{w_j} \leq l
\end{split}
\end{equation}

Here, $\srob_{\varphi_j}$ is the smooth robustness, and $L$ is a 
linear map that takes a sequence of waypoints $\mathbf{w}_j$ (vectors 
in 3D position and velocity space) to generate a discrete-time 
trajectory $\sstraj_j=L(\mathbf{w}_j)$ of duration $hrz(\varphi_j)$. 
This trajectory consists of spline segments that minimize the 
integral of jerk over time going from one waypoint to the next 
\cite{MuellerTRO15}. The linear constraints on the waypoints are such 
that they ensure kinematic feasibility (Theorem 3.2 in 
\cite{pant2018fly}) of the resulting trajectories, i.e. the 
velocities and accelerations of the UAS are within predefined bounds. 
For brevity , we omit the details here, but the full formulation can 
be found in \cite{pant2018fly}. The resulting robustness value of the 
generated trajectory $\sstraj_j$, $\rho_{\varphi_j}$, defines the 
robustness tube around the trajectory. 

By allowing each UAS to plan for itself independent of the others, we have ignored the mutual separation requirement in the STL-based planning problem. Instead we rely on online collision avoidance to pairwise ensure that UAS do not crash with each other. This is covered in the following section.

\textbf{Note:} In the following sections, $\mathbf{x}$ will refer to a full-state (discrete-time, finite duration) trajectory for a UAS. We will also use $\mathbf{p}$ to refer to the position components in that trajectory, or the position trajectory. $x_k$ (and $p_k$) refer to the components of the trajectory at time step $k$.

%The robustness value $\rho_d*$ achieved through solving this optimization can be interpreted as a discrete tube in the position space $P_d$ such that as long as the discrete time positions of the UAS remain inside the robustness cubes of size $2\rho_d$ centered around the planned positions, $\phi_d$ is satisfied (see Theorem \ref{thm:rob objective}). See fig \ref{fig:concept} for a visualization of this interpretation. It should be noted that such a trajectory (and its robustness tube) can be generated by other methods as well, e.g. that of \cite{Raman14_MPCSTL}, but we use \cite{pant2018fly} because of it being computationally faster and tailored for multi-rotor robots.
